Overall Complexity Certification of a Standard Branch and Bound Method for Mixed-Integer Quadratic Programming

This paper presents a method to certify the computational complexity of a standard Branch and Bound method for solving Mixed-Integer Quadratic Programming (MIQP) problems defined as instances of a multi-parametric MIQP. Beyond previous work, not only the size of the binary search tree is considered, but also the exact complexity of solving the relaxations in the nodes by using recent result from exact complexity certification of active-set QP methods. With the algorithm proposed in this paper, a total worst-case number of QP iterations to be performed in order to solve the MIQP problem can be determined as a function of the parameter in the problem. An important application of the proposed method is Model Predictive Control for hybrid systems, that can be formulated as an MIQP that has to be solved in real-time. The usefulness of the proposed method is successfully illustrated in numerical examples.

==> complex_cert_full_alg.tex <==
	\section{Complexity certification of MIQP} \label{sec:cert}
	In this section, we study how Algorithm \ref{alg1} behaves for various values of the parameter $\theta$. 
	Note that in a hybrid MPC, these parameters could be system states or\slash and reference signals. %The pre-computed mp-MIQPs are then stored in a look-up table, which is then evaluated online for a specific parameter. 
	The following definitions are useful in analyzing the parametric properties.
		
	\begin{definition} \label{def1}	
	A set of polyhedra $\mathcal{R}_i, \hspace{.01cm} i=1,...,N$ is a polyhedral partition of $\Theta$ if  $ \mathcal{R}_i \cap \mathcal{R}_j = \emptyset, i\neq j$, and $\cup_{i=1}^{N} \mathcal{R}_i = \Theta$.
	\end{definition} 	
	
	\begin{definition} \label{def2}	
	A function $x(\theta): \Theta \rightarrow  \mathbb{R}^n$, where $\Theta \subset  \mathbb{R}^n$ is a polyhedral set, is piecewise affine (PWA) if it is possible to partition $\Theta$ into convex polyhedral regions $\mathcal{R}_i$, and $x(\theta) = H_i \theta + K_i, \hspace{.1cm} \forall  \theta \in  \mathcal{R}_i$.	
	\end{definition} 

	Note that if $\mathcal{R}_i$s are convex polyhedral regions, then PWA function $x(\theta)$ is called polyhedral piecewise affine (PPWA). 
	Piecewise quadratic functions (PWQ) and polyhedral piecewise quadratic functions (PPWQ) are defined, analogously.

	%	% \textbf{Theorem 1} (Properties of mp-QP solution \cite{c6}): \label{theorem1}	
	%	% Consider the mp-QP in \eqref{eq4} and let $H \in \mathbb{S}_{+}^n$, and  $\Theta$ be convex. Then the set of feasible parameters  $\Theta^* \subseteq \Theta$ is convex, the optimizer $x^*(\theta)$ is continuous and PPWA, and the optimal objective function $J^*(\theta)$ is continuous, convex and PPWQ. 	
	%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	To certify an MIQP, iterations of Algorithm \ref{alg1} are executed parametrically with respect to $\theta$, for a given set $\Theta$ of parameters. If the intention is to find the total number of relaxations encountered in the tree, the certification is fulfilled by solving mp-QPs %in Step \ref{alg2_cert}
	and incrementally increasing the complexity measure at each outer iteration of B\&B. A QP certification method is employed otherwise at each node for which each computation partitions the parameter space into polyhedral regions. Exploring the search tree leads to certifying a sequence of mp-QPs which each partitions the parameter space into different regions and keeping track of the complexity measure at each parameter could become challenging. One possibility would be to find the intersection between regions and then summing up the complexity measure corresponding to the intersected regions. This approach results in non-polyhedral regions which increases the computational complexity when going down in the search tree. In this paper, the branch and bound is modified to avoid the necessity of finding intersection between regions, while the complexity measures resulted from certifying the relaxations are summed when reaching to optimal integer solution in each parameter. 
	Note that in this work, the parameter space is partitioned based on the solver state, not based on the explicit solution. Explicit solution is technically a by-product of our analysis.	
	
	Algorithm \ref{alg2} represents the proposed parametric B\&B with the aim of certifying MIQP problem \eqref{eq3} in detail. 
	Here, $\kappa(\theta)$ denotes a complexity measure for solving the QP relaxation \eqref{eq4} denoted by $\mathcal{P}(\theta,\mathcal{B}_0,\mathcal{B}_1)$.		
	In addition to the usual stack $\mathcal{T}$ of B\&B, there are two additional stacks of tuples in Algorithm \ref{alg2}. One is stack $\mathcal{S}$ holding regions where the analysis has not completed yet. 
	It contains tuples $\left ( \Theta,\kappa,\mathcal{T},\bar{\mathbb{J}}(\theta) \right )$, where $\Theta$ is the associated polyhedral parameter set, $\mathcal{T}$ is the normal stack of B\&B to store subproblems, $\kappa$ is a complexity number, and $\bar{\mathbb{J}}(\theta)$ is a collection of the upper bounds on the value function. Another stack is $\mathcal{F}$ which holds terminated regions building the final partition. 
	It consists of a tuple with the information $(\Theta,\kappa)$ for every terminated region with the associated complexity measure. 
		
	The function $\textsc{QPcertification} \left (\mathcal{P}(\theta,\mathcal{B}_0,\mathcal{B}_1),\Theta \right )$ is the complexity certification routine for QPs which takes as an input an mp-QP problem $\mathcal{P}(\theta,\mathcal{B}_0,\mathcal{B}_1)$ and a parameter region $\Theta$ and returns a partition $\{\Theta^j\}_{j=1}^{N}$ of $\Theta$. In each region, the function provides the computational complexity $\kappa^j$ for solving $\mathcal{P}(\theta,\mathcal{B}_0,\mathcal{B}_1)$ for all parameters in $\Theta^j$, as well as the optimal active set $\mathcal{A}^j$ and the value function $J^j(\theta)$ which is PPWQ, i.e., convex piecewise quadratic over the polyhedral region.  
	If $\mathcal{P}(\theta)$ is infeasible in $\Theta^j$, we set $J^j(\theta)=\infty$.
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	There is a freedom in the choice of complexity measure and Algorithm \ref{alg2} is not restricted to a specific certification function. If the QP certification in \cite{arnstrom2021unifying} is employed on Line \ref{alg2_cert},  
	then the complexity measure $\kappa^j$ will be the iteration number, that is the total number of linear system equations that have to be solved, i.e., the number of equality constrained QPs that an active-set method requires to solve to reach the optimal solution. 
	Another alternative is to fix $\kappa^j$ to $1$. Then the complexity measure will be the total number of nodes required to be explored in the B\&B tree, i.e., the number of relaxations. The other important choice is if $\kappa^j$ holds the number of floating point operations (flops) for solving the QP, given by the QP certification algorithm. It then results in the total number of operations performed to solve all the relaxations in B\&B.
	
	Properties of the proposed certification method are discussed in more detail in the following subsections.
		
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{algorithm}[H]
		\caption{Certification of Branch and Bound for MIQP} 
		\label{alg2}
		\hspace*{\algorithmicindent} \textbf{Input}: mp-MIQP problem $\mathcal{P}(\theta)$, and $\Theta_0$ \\ 
		\hspace*{\algorithmicindent} \textbf{Output}: final partition $\mathcal{F}$	
		\begin{algorithmic}[1] 
			%\Statex
			\STATE $ \bar{J} \leftarrow \infty$ %, $\bar{x} \leftarrow $ void
			\STATE $\kappa_0 \leftarrow 0$, $\mathcal{F} \leftarrow \emptyset $
			\STATE $ \bar{\mathbb{J}} \leftarrow \bar{J}$  
			\STATE{Push $\mathcal{P} \left (\theta, \emptyset, \emptyset \right )$ to $\mathcal{T}_0$}
			\STATE Push $(\Theta_0, \kappa_0, \mathcal{T}_0,\bar{\mathbb{J}})$ to $\mathcal{S} $ %,\bar{x}
			\WHILE {$\mathcal{S} \neq \emptyset$}
			\STATE Pop $ \left ( \Theta,\kappa, \mathcal{T},\bar{\mathbb{J}}(\theta)  \right )$ from $\mathcal{S} $ %,\bar{x}(\theta) 
			\IF {$\mathcal{T}=\emptyset$}
			\STATE Push $(\Theta,\kappa)$ to $\mathcal{F}$ 
			\ELSE
			\STATE Pop $\mathcal{P} \left ( \theta,\mathcal{B}_0,\mathcal{B}_1 \right )$ from  $\mathcal{T}$ \label{alg2_pop}
			\STATE $\{(\Theta^j, \kappa^j, \mathcal{A}^j, J^j(\theta))\}_{j=1}^N \leftarrow$ \\ $\hspace{1.6cm} \textsc{QPcertification}\left ( \mathcal{P}(\theta,\mathcal{B}_0,\mathcal{B}_1),\Theta \right )$ \\
			\label{alg2_cert} %, x^j(\theta), 
			\FOR{$j\in\{1,\dots,N\}$} \label{alg2_for}
			\STATE $\mathcal{T}^j \leftarrow$  $\mathcal{T}$ %copy
			\STATE $\bar{\mathbb{J}}^j(\theta) \leftarrow$  $ \bar{\mathbb{J}}(\theta)$ 
			\IF {$ \exists \bar{J} \in \bar{\mathbb{J}}^j$ : $ J^{j}(\theta) \geq \bar{J}(\theta)$, $\forall \theta\in \Theta^j$} 
			\label{alg2_comp}	
			\STATE There exists no $\theta$ for which a feasible solution of $\mathcal{P}$  provides better solution %than $\bar{x}(\theta) $  
			\ELSIF {all binary variables are in $\mathcal{A}^j$}  \label{alg2_feas}
			%\Comment{\textcolor{blue}{integer feas. cut}}
			\STATE  Potentially better integer feasible solution has been found % for a subset of the parameter space
					\STATE $\bar{\mathbb{J}}^j(\theta) \leftarrow$   $\left\{\begin{matrix}
					J^j(\theta)
					\\ 
					\bar{\mathbb{J}}^j(\theta)
					\end{matrix}\right.$ 
			\ELSE				
			\STATE Select $k$ : $k \in \mathcal{B}$, $k \notin (\mathcal{B}_0 \cup \mathcal{B}_1) $ 
			\STATE Push $\mathcal{P}(\theta,\mathcal{B}_0 \cup \{k\},\mathcal{B}_1)$ and $\mathcal{P}(\theta,\mathcal{B}_0,\mathcal{B}_1 \cup \{k\})$ to $\mathcal{T}^j$ 
			\ENDIF
			\STATE Push $ \left (\Theta^j,\kappa+\kappa^j,\mathcal{T}^j,\bar{\mathbb{J}}^j(\theta) \right )$ to $\mathcal{S}$ \label{alg2_increase} %,\bar{x}^j(\theta) 
			\ENDFOR
			\ENDIF
			\ENDWHILE
		\end{algorithmic}
	\end{algorithm}
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	\begin{algorithm}[H]
%		\caption{Parametric certification method}
%		\label{alg:bnbcert}
%		\begin{algorithmic}[1]
%			\Require mp-MIQP problem, parameter region $\Theta_0$ 
%			\Ensure Partition $\mathcal{F}=\{(\Theta^i,\kappa^i)\}_{i=1}^{N_f}$ 
%			\State $\kappa_0 \leftarrow 0$; $\mathcal{T}_0 \leftarrow \{\emptyset, \emptyset\}$; $\bar{\mathbb{J}}_0 \leftarrow \{\infty\}$
%			\State $\mathcal{F} \leftarrow \emptyset$
%			\State Push $(\Theta_0, \kappa_0, \mathcal{T}_0, \bar{\mathbb{J}}_0)$ to $S$
%			\algrenewcommand\algorithmicindent{0.8em}%
%			\While{$S\neq \emptyset$}\label{step:outer-loop}
%			\State $(\Theta,\kappa,\mathcal{T},\bar{\mathbb{J}}) \leftarrow $ pop from $S$   
%			\If {$\mathcal{T}=\emptyset$}
%			\State Push $(\Theta,\kappa)$ to $\mathcal{F}$ and \textbf{goto} Step \ref{step:outer-loop}\label{step:add-to-final}
%			\EndIf
%			\State $(\mathcal{B}_0,\mathcal{B}_1) \leftarrow$ pop from $\mathcal{T}$
%			\State $\left\{\left(\Theta^i,\kappa^i,\mathcal{A}^i, J^{*i}\right)\right\}_{i=1}^N \leftarrow$ solve $\mathcal{P}(\theta,\mathcal{B}_0, \mathcal{B}_1)$ over $\Theta$ \label{step:solve-relaxation}
%			\For{$i \in \{1,\dots, N\}$}  
%			\State $\mathcal{T}^i, \bar{\mathbb{J}}^i \leftarrow \textsc{updateTree}(\mathcal{T},\mathcal{A}^i, J^i,\bar{\mathbb{J}})$ 
%			\State Push $(\Theta^i,\kappa+\kappa^i,\mathcal{T}^i, \bar{\mathbb{J}}^i)$ to $S$ 
%			\EndFor
%			\EndWhile
%		\end{algorithmic}
%	\end{algorithm}
	%%%%%%%%%%%%%%%%%%%%%% Cutting parametric Bnb tree%%%%%%%%%%%%%%%%
	\subsection{Spatial Decomposition} \label{subsec:spatial-decom} 
	In the parametric search tree, some spatial splitting in addition to the usual splitting a node into two new subproblems in B\&B for exploring the tree are applied.
	The spatial decomposition first occurs from Step \ref{alg2_cert} to split a node into the subproblems with smaller regions after certifying an mp-QP. Each node with a new finer region $\Theta^j$ will be then the root node of a local tree that follows after. The result of this analysis is many local trees, which would be all possible B\&B trees that are used to compute the solution of the problem for all parameter values, online.
	
	The usual B\&B procedure, e.g., searching for the cut conditions, then applies for every local tree. %and consequently the three cut conditions of B\&B are imposed. 
	The infeasibility and integer feasibility cut conditions will directly be given from what is outputted in $\textsc{QPcertification} \left (\mathcal{P}(\theta,\mathcal{B}_0,\mathcal{B}_1),\Theta \right)$, given by $J^j(\theta)=\infty$ and the active set $\mathcal{A}^j$ for the region, respectively, with no further spatial partitioning. In the dominance cut however, if it is done exactly, further spatial partitioning is imposed by $ J^{j}(\theta) \geq \bar{J}(\theta)$ to split the node into two new subproblems with regions where the comparison holds and not. % $\forall \theta\in \Theta^j$. 
	To make the certification more tractable, at the price of conservatism, the spatial partitioning stemming from the dominance cut can be avoided by only cutting if $ J^{j}(\theta) \geq \bar{J}(\theta)$, $\forall \theta\in \Theta^j$. % for all $\theta$ in the new region.	
	
	%%%%%%%%%%%%%%%%%%%%%% Cutting parametric Bnb tree%%%%%%%%%%%%%%%%
	\subsection{Parametric cut conditions} \label{subsec:param-cut-conditions} 
	The pruning done in Algorithm \ref{alg2} for each node $j$ are implied as follows. If the cut condition on Line \ref{alg2_comp}, which searches for both infeasibility and dominance criterion simultaneously, holds, then there will not be any parameter for which an online algorithm would have continued. 
	Otherwise, the integer feasibility cut condition is checked on Line \ref{alg2_feas}. If the solution is integer feasible in the corresponding parameter set, meaning that the binary constraints are active in the active set $\mathcal{A}^j$, then the objective function value is appended to the upper bound. As a result, the upper bound $\bar{\mathbb{J}}(\theta)$ is the ponitwise minimizer of 
	 a collection of value functions corresponding to integer feasible solutions found from the parametric relaxations encountered so far.  

	If any of the above cut conditions holds, the tree is cut, otherwise the tree is branched on the corresponding parameter set resulting in two new nodes which are pushed in the stack $\mathcal{T}^j$ for further analysis. 	
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\subsection{Properties of the search tree}	\label{subsec:prop of tree}
	The parametric upper bound in a node for each parameter value is required to coincide with the upper bound an online solver would use in that node for each $\theta$. To guarantee that, the following assumption is made.
	
	\begin{assumption} \label{assumption-order-tree}
		%The exploration tree in $\mathcal{T}$ for the analysis in Algorithm \ref{alg2} and the online solver in Algorithm \ref{alg1} is depth-first. Moreover, the  %The order in which the analysis in Algorithm \ref{alg2} and the online solver in Algorithm \ref{alg1} explore the tree in $\mathcal{T}$ are the same. % for all parameter values.
		The tree exploration strategy is depth first in Algorithms \ref{alg1} and \ref{alg2}. Moreover, the branch variable order is fixed
		(e.g., not parameter dependent) and known beforehand, and the order in which the $0$ and $1$ branch will be explored is fixed and known beforehand in the both algorithms.
	\end{assumption}
	
	Let a \textit{node} be donated by tuple $\eta \triangleq (\mathcal{B}_0, \mathcal{B}_1)$, where $\mathcal{B}_0$ and $\mathcal{B}_1$ are defined in \eqref{eq4}. The following definition then can be applied for B\&B algorithms. 
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{definition} \label{descendent}	
	 The node $\eta=(\mathcal{B}_0, \mathcal{B}_1)$ is \textit{descendant} to node $\hat{\eta}=(\hat{\mathcal{B}}_0, \hat{\mathcal{B}}_1)$, denoted by  $\eta\in\mathcal{D}(\mathcal{\hat{\eta}})$, if $\mathcal{B}_0 \supseteq \hat{\mathcal{B}}_0$ and $\mathcal{B}_1 \supseteq \hat{\mathcal{B}}_1$. 
	\end{definition}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	To state the properties of the certification algorithm, the following Lemma is needed.
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{lemma}
		\label{lem:dominance-parent}
		Let $J^*_{\eta}(\theta)$ denote the value function for the mpQP in node $\eta$ and let $\delta \in \mathcal{D}(\eta)$, then $J^*_{\eta}(\theta)\leq J_{\delta}^*(\theta)$. 
	\end{lemma}
	\begin{proof}
		It directly follows from the feasible set for the mp-QP in node $\delta$ which is a subset of the feasible set for the mpQP in node $\eta$, as some inequality constraints in $\eta$ are imposed to hold with equality in $\delta$. 
	\end{proof}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	Let $\mathbb{B}_\eta(\theta)$ be the set of nodes which have yielded an integer feasible solution up until node $\eta$ is processed, given an ordering of $\mathcal{T}$. Moreover, let $\bar{J}_{\eta}(\theta)$ denote the lowest upper bound found up until $\eta$ is processed, i.e., 
	\begin{equation}
	\bar{J}_{\eta}(\theta) \triangleq \min_{\tilde{\eta}\in\mathbb{B}_{\eta}(\theta)} J^*_{\tilde{\eta}}(\theta). 
	\end{equation}
	
	The following lemma shows that if the dominance cut condition is invoked for node $\eta$, the best upper bound $\bar{J}_{\eta}(\theta)$ will not be changed by processing descendants of $\eta$. 
	\begin{lemma}
		\label{lem:redundant-desc}
		Assume that $J^*_{\eta}(\theta)\geq \bar{J}_{\eta}(\theta)$, that is the dominance cut will be invoked. Then 
		\begin{equation}
		\min_{\tilde{\eta}\in \mathbb{B}_{\eta}(\theta)\cup \mathcal{D}(\eta)} J^*_{\tilde{\eta}}(\theta) = \bar{J}_{\eta}(\theta).
		\end{equation}
	\end{lemma}
	\begin{proof}
		We have that  
		\begin{equation*}
		\begin{aligned}
		\min_{\tilde{\eta}\in \mathbb{B}_{\eta}(\theta)\cup \mathcal{D}(\eta)} J^*_{\tilde{\eta}}(\theta) 
		&= \min\left\{\min_{\tilde{\eta}\in\mathbb{B}_{\eta}(\theta)}J^*_{\tilde{\eta}}(\theta),\min_{\delta\in \mathcal{D}(\eta)} J_{\delta}^*(\theta) \right\} \\
		&= \min\left\{\bar{J}_{\eta}(\theta), \min_{\delta\in \mathcal{D}(\eta)} J_{\delta}^*(\theta) 
		\right\} \\
		&= \bar{J}_{\eta}(\theta),
		\end{aligned}
		\end{equation*}
		where the last equality follows from $J_{\delta}^*(\theta)\geq J_{\eta}^*(\theta) \geq \bar{J}_{\eta}(\theta)$ $\forall\delta\in \mathcal{D}(\eta)$, i.e., from Lemma \ref{lem:dominance-parent} and the premise. 
	\end{proof}
	Hence, processing descendants of a node for which the dominance cut was invoked would not change the best upper bound. In other words, the exploration of the rest of the tree will not be affected if $\mathcal{T}\cup D(\eta)$ is used instead of $\mathcal{T}$ after the dominance cut is invoked in node $\mathcal{\eta}$. We formalize this notion in the following corollary:
	
	\begin{corollary}
		\label{cor:redundant-desc-exploration}
		Consider two cases of the list $\mathcal{T}$ after the dominance cut is invoked when processing node $\eta$
		\begin{enumerate}
			\item $\mathcal{T}$ is used (normal operation) 
			\item $\mathcal{T}\leftarrow \mathcal{T}\cup \mathcal{D}(\eta)$ is used (redundant addition) 
		\end{enumerate}
		Let $\mathbb{B}^1$ be the set of \textit{all} nodes explored during case 1 and let $\mathbb{B}^2$ be the set of \textit{all} nodes explored during case 2. Then $\mathbb{B}^2 \setminus \mathbb{B}^1 = \mathcal{D}(\eta)$. That is, exploring the nodes in $\mathcal{D}(\eta)$ does not affect the subsequent exploration of nodes in the tree. 		
	\end{corollary}
	\begin{proof}
		The only thing that might alter the exploration is if the upper bound is changed by processing additional nodes (which could prune nodes that would otherwise be explored). However, from Lemma \ref{lem:redundant-desc} processing any descendants of $\eta$ can never change the best upper bound, which in turn means that further exploration is unaffected by processing any $\delta \in \mathcal{D}(\eta)$.
	\end{proof}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%	\begin{corollary}
	%		\label{cor:redundant-desc-exploration}
	%		Consider two cases of the list $\mathcal{T}$ after the dominance cut is invoked when processing node $\eta$
	%		\begin{enumerate}
	%			\item $\mathcal{T}$ is used (normal operation) 
	%			\item $\mathcal{T}\leftarrow \mathcal{T}\cup \mathcal{D}(\eta)$ is used (redundant addition) 
	%		\end{enumerate}
	%		Let $\mathbb{B}^1$ be the set of \textit{all} nodes explored during case 1 and let $\mathbb{B}^2$ be the set of \textit{all} nodes explored during case 2. Then $\mathbb{B}^2 \setminus \mathbb{B}^1 = \mathcal{D}(\eta)$. That is, exploring the nodes in $\mathcal{D}(\eta)$ does not affect the subsequent exploration of nodes in the tree. 
	%		
	%	\end{corollary}
	%	\begin{proof}
	%		The only thing that might alter the exploration is if the upper bound is changed by processing additional nodes (which could prune nodes that would otherwise be explored). However, from Lemma \ref{lem:redundant-desc} processing any descendants of $\eta$ can never change the best upper bound, which in turn means that further exploration is unaffected by processing any $\delta \in \mathcal{D}(\eta)$.
	%	\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Properties of the certification}	\label{subsec:prop of cert}	
	In this subsection, the properties of the proposed certification method are derived.
	\begin{theorem}	 \label{theorem-sequence} 
		Assume Assumption \ref{assumption-order-tree} holds. %Then the sequence of nodes explored by Algorithm \ref{alg1} is a subsequence of the sequence of explored nodes by Algorithm \ref{alg2}.
		Let $\mathbb{B}(\theta)$ denote the set of all the nodes that are explored to solve the MIQP in \eqref{eq5} given $\theta$ using the B\&B algorithm in Algorithm \ref{alg1}. Moreover, let $\hat{\mathbb{B}}_k(\theta)$ denote all nodes that were explored in Algorithm \ref{alg2} for region $\Theta_k$ before terminating. Then $\mathbb{B}(\theta) \subseteq \hat{\mathbb{B}}_k(\theta)$, $\forall \theta\in \Theta_k$.
	\end{theorem}
	\begin{proof} \label{proof-theorem-sequence}  
		Consider the processing of node $\eta$ on region $\Theta$ in Algorithm \ref{alg2} and assume that a conservative upper bound $\tilde{J}(\theta)$ on $\Theta$ is used for the dominance cut (i.e., $\tilde{J}(\theta)\geq \bar{J}_{\eta}(\theta), \forall \theta\in \Theta$). Then we have the following cases:
		\begin{enumerate}
			\item $J^*_{\eta}(\theta) \geq \tilde{J}(\theta)$ $\forall \theta\in \Theta$ $\rightarrow$ dominance cut invoked correctly $\forall\theta \in \Theta$. 
			\item $\exists \tilde{\theta}\in \Theta$ such that $ J^*_{\eta}(\tilde{\theta}) <   \tilde{J}(\theta)$ 
			\begin{enumerate}
				\item $J^*_{\eta}(\theta) < \bar{J}_{\eta}(\theta)$ $\forall \theta\in \Theta$ $\rightarrow$ dominance cut dismissed correctly for all $\theta \in \Theta$. 
				\item Otherwise dominance cut is dismissed incorrectly for all $\theta\in\Theta^{\epsilon}\triangleq\{\theta\in \Theta: J_{\eta}^*(\theta) \geq \bar{J}_{\eta}(\theta)\}$
			\end{enumerate}
		\end{enumerate}
		
		The most critical situation is in 2b), where we might explore descendants to $\eta$ in the certification algorithm, while these would be pruned in Algorithm 1 pointwise. 		
		The possible extra nodes in the analysis are pushed in the $\mathcal{T}^k$ according to Assumption \ref{assumption-order-tree} and consequently, when a new node  is popped from the stack in Step \ref{alg2_pop} of Algorithm \ref{alg2} to be analyzed, it is either the relevant one that would be solved in the online solver for a specific parameter in the corresponding region, or redundant which has been cut away in Algorithm \ref{alg1}. For parameters with redundant considerations where the error in 2b) happens, we have that $J^*_{\eta}(\theta)\geq \bar{J}_{\eta}(\theta)$. According to Corollary \ref{cor:redundant-desc-exploration}, the extra exploration of descendants to $\eta$ will not affect the other exploration. Therefore, $ \hat{\mathbb{B}}_k(\theta) \supseteq \mathbb{B}(\theta)$, $\forall \theta\in \Theta_k$.
	\end{proof}
	 
	 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\begin{theorem} \label{cor-conserve-cert}	%(Complexity certificates): 
 	Assume Assumption \ref{assumption-order-tree} holds and assume that a conservative upper bound $\bar{J}(\theta)$ on $\Theta$ is used for the dominance cut %(i.e., $\tilde{J}(\theta)\geq \bar{J}_{\eta}(\theta), \forall \theta\in \Theta$) 
 	in Step \ref{alg2_comp} of Algorithm \ref{alg2}. Let $\kappa(\theta)$ be a complexity measure for solving the QP relaxation $\mathcal{P}(\theta)$ returned by $\textsc{QPcertification} \left ( \mathcal{P}(\theta),\Theta \right )$ and that it satisfies $\kappa^j = \kappa(\theta)$, $\forall \theta\in \Theta^j \subseteq \Theta $, $\forall j$. Moreover, let $\{\Theta^i, \kappa^i_{tot} \}_{i=1}^{N_{\mathcal{F}}}$ be the collection of tuples in  $\mathcal{F}$ returned by Algorithm \ref{alg2} and let $\kappa^*_{tot}(\theta)$ be the total complexity for solving all QP relaxations encountered in Algorithm \ref{alg1} for $\theta \in \Theta_0 $. Then $\kappa^i_{tot} \geq \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$.
 	\end{theorem}
 	\begin{proof} \label{proof-cor-conserve-cert} 
 	Based on the result from Theorem \ref{theorem-sequence}, the QP relaxations that are considered in Algorithm \ref{alg2} for a single point $\tilde{\theta}$ will be a superset of the QP relaxations that would be solved in Algorithm \ref{alg1}. This in turn means that the total complexity $\{\kappa^i_{tot}\}_{i}$ returned by Algorithm 2 will be an upper bound on the total complexity of Algorithm 1 (pointwise), i.e., $\kappa^i_{tot} \geq \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$.   
 	%It immediately results from Theorem \ref{theorem-exact} and Theorem \ref{theorem-conservative}, such that in the actual PPWQ function comparisons, based on Theorem \ref{theorem-exact} , $\kappa^i_{tot} = \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$ whereas based on Theorem \ref{theorem-conservative}, $\kappa^i_{tot} \geq \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$, otherwise. %\qed
 	\end{proof}
	 
	 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	 \begin{corollary}	 \label{cor-exact-cert} %(Complexity certificates):
	 	Assume Assumption \ref{assumption-order-tree} holds. Moreover assume that the comparison of value functions $J^j(\theta)$ with the upper bound $\bar{J}(\theta)$ on $\Theta^j$ in Step \ref{alg2_comp} of Algorithm \ref{alg2} is exact. Let the collection of tuples $\{\Theta^i, \kappa^i_{tot} \}_{i}$ and $\kappa^*_{tot}(\theta)$ be defined as in Corollary \ref{cor-conserve-cert}. Then $\kappa^i_{tot} = \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$. %Let regions be treated as atomic unit. Then the proposed complexity certification results can be somewhat conservative.
	 \end{corollary}
 	\begin{proof}  \label{proof-cor-exact-cert} %(Complexity certificates):
 		 Consider the pruning done in Step \ref{alg2_comp} in Algorithm \ref{alg2}. If the comparison $\tilde{\theta} \in \Theta^k$ is done exactly, the situation in the step 2b), stated in the proof of Theorem \ref{theorem-sequence}, would never happen. According to the reasoning in Theorem \ref{theorem-sequence}, it then means that $\mathbb{B}(\theta) = \hat{\mathbb{B}}_k(\theta)$, $\forall \theta\in \Theta_k$, where $\hat{\mathbb{B}}_k(\theta)$ and $\hat{\mathbb{B}}_k(\theta)$ are defined in Theorem \ref{theorem-sequence}. As the same set of nodes are explored in the analysis and the online solver, the obtained complexity measure from Algorithm \ref{alg2} coincides with the Algorithm \ref{alg1}. 	
 	\end{proof}
 	
 	Note that the actual comparison results in quadratic cuts in the partitions which would make the final partition non-polyhedral. On the other hand, by approximate comparison, there might be a non-zero gap between the measured complexity of the Algorithm \ref{alg2} with the online solver for a specific point. However all regions remain polyhedral which makes the computations significantly cheaper. So, there is a trade-off between computational time and the accuracy of the analysis. 
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	\begin{theorem}	 \label{theorem-exact} %(Exact complexity certificates)
%	Assume Assumption \ref{assumption-order-tree} holds. Moreover assume that the comparison of value functions $J^j(\theta)$ with the upper bound $\bar{J}(\theta)$ on $\Theta^j$ in Step \ref{alg2_comp} of Algorithm \ref{alg2} is exact. Let $\kappa(\theta)$ be a complexity measure for solving the QP relaxation $\mathcal{P}(\theta)$ returned by $\textsc{QPcertification} \left ( \mathcal{P}(\theta),\Theta \right )$ and that it satisfies $\kappa^j = \kappa(\theta)$, $\forall \theta\in \Theta^j \subseteq \Theta $, $\forall j$. Moreover, let $\{\Theta^i, \kappa^i_{tot} \}_{i}$ be the collection of tuples in  $\mathcal{F}$ returned by Algorithm \ref{alg2} and let $\kappa^*_{tot}(\theta)$ be the total complexity for solving all QP relaxations encountered in Algorithm \ref{alg1} for $\theta \in \Theta_0 $. Then $\kappa^i_{tot} = \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$. %then the complexity certification result coincides with the complexity of the online solver for each parameter in parameter space. %$\kappa^i_{tot} = \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$.
%	\end{theorem}
%	\begin{proof} \label{proof-theorem-exact} 
%	Algorithm \ref{alg2} applies Algorithm \ref{alg1} to all parameters, while keeping track of the complexity measure for each parameter. %So as discussed, % in the previous subsection, 
%	%studying the cut conditions are performed parametrically 
%	Parametric cut conditions of Algorithm \ref{alg2} in Steps \ref{alg2_comp} and \ref{alg2_feas} correspond to Steps \ref{alg1-cut2} and \ref{alg1-cut3} of Algorithm \ref{alg2} for a specific parameter, respectively. Consider the pruning done in Step \ref{alg2_comp} in Algorithm \ref{alg2}. This pointwise comparison is equivalent to solving the following minimization problem
%	\begin{align} \label{eq6-2} 
%	%\vspace{.1cm} 
%	\min_{\theta  \in \Theta^j } \Delta J =  \quad &  \min_{\theta  \in \Theta^j } J^{j}(\theta) - \bar{J}(\theta) 		
%	\end{align} 
%	The exact comparison of the value function of relaxation with the upper bound divides the region $\Theta^j$ to two finer regions %  $ J^{j}(\theta)$ %$\bar{J}(\theta)$
%	\begin{equation}
%		\begin{aligned} \label{eq7} 
%		%\vspace{.1cm} 
%		\Theta ^{j_1} = \quad & \Theta ^{j} \cap (\Delta J \geq 0)  \\ 
%		\Theta ^{j_2} = \quad & \Theta ^{j} \cap (\Delta J \leq 0)			
%		\end{aligned}
%	\end{equation}
%	The offline tree is cut for the region $\Theta ^{j_1}$, while it continues traversing the tree, i.e., searching for the integer feasibility, 
%	in the region $\Theta ^{j_2}$. That is, for parameters that the value function of relaxation is worse than the upper bound, there will be no branching. The same is occurred  in Algorithm \ref{alg1} in which for $\forall \tilde{\theta} \in \Theta ^{j_1}$, the online tree is pruned in Step \ref{alg1-cut2}. However, it tests the next cut condition for $\forall \tilde{\theta} \in \Theta ^{j_2}$, as $\tilde{J} \leq \bar{J}$, where $\tilde{J}$ is the value function of the relaxation for $\tilde{\theta} \in \Theta ^{j_2}$. The upper bound is then updated for $\theta \in \Theta ^{j_2}$ if the solution is integer feasible in Step \ref{alg2_feas} and Step \ref{alg1-cut3} of Algorithm \ref{alg2} and Algorithm \ref{alg1}, respectively. Otherwise the tree is branched in that node for the both algorithms. %TODO: add more argument here
%	Under the assumption of theorem, it results that the same sequence of nodes are explored in the analysis and in the online computing. %sequence of nodes that explored in the analysis is identical to the sequence of explored nodes in online computing.
%	Since the same relaxation problems are solved in the both algorithms, the complexity measure from the analysis and the online solver coincides for all parameters. As a result, the proposed complexity certification for MIQP is exact.  %\qed
%	%In comparing the value function of the relaxation $ J^{j}(\theta)$ with the value function of the parametric upper bound $\bar{J}(\theta)$ in Step \ref{alg2_comp}, any algorithm that supports non-convex partitions could be used. Such comparison results in non-polyhedral regions which cause no overlap in the upper bound and the search tree is branched just for the parameters in $\Theta^j$ that satisfies $J^j(\theta) < \bar{J}(\theta)$, and is cut for the rest of $\theta\in \Theta^j$, otherwise. 
%	%In this way, the sequence of nodes that are visited in the offline tree is identical to the one in the online solver. As the same nodes are seen and solved in both solver, for each specific parameter, the same QP relaxation is solved and as a result, the proposed complexity certification for MIQPs is exact.  \qed %, i.e., $\kappa^i_{tot} = \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$.  \qed
%	\end{proof}
%		
%	Note that the actual comparison results in quadratic cuts in the partitions which would make the final partition non-polyhedral. %$\forall \theta\in \Theta^j$,	
%	To circumvent that, the following consideration can be applied. 
%	
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	\begin{theorem}	 \label{theorem-conservative} %(Complexity certificates):
%	Assume Assumption \ref{assumption-order-tree} holds and assume that a conservative upper bound $\bar{J}(\theta)$ on $\Theta$ is used for the dominance cut %(i.e., $\tilde{J}(\theta)\geq \bar{J}_{\eta}(\theta), \forall \theta\in \Theta$) 
%	in Step \ref{alg2_comp} of Algorithm \ref{alg2}. Let the collection of tuples $\{\Theta^i, \kappa^i_{tot} \}_{i}$ and $\kappa^*_{tot}(\theta)$ are defined as in Theorem \ref{theorem-exact}. Then $\kappa^i_{tot} \geq \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$. %Let regions be treated as atomic unit. Then the proposed complexity certification results can be somewhat conservative.
%	\end{theorem}
%	\begin{proof} \label{proof-theorem-conservative}  
%	In comparing the value function of the relaxation $ J^{j}(\theta)$ with the value function of the parametric upper bound $\bar{J}(\theta)$ in \eqref{eq6-2}, to avoid non-polyhedral regions, the tree is cut only when the comparison holds in the entire domain, i.e., $\delta \theta _{min} \geq 0$, where $\delta \theta _{min}$ is the solution of \eqref{eq6-2}. 
%	
%	Consider a region $\Theta^k$ with the complexity measure $\tilde{\kappa}$ in which $\delta \theta _{min} < 0$.  %, k \in\{1,\dots,N\} %\tilde{\kappa}%\kappa^k
%	Let $\tilde{\theta} \in \Theta^k$ be a point for which the $J^{k}(\tilde{\theta}) > \bar{J}(\theta), \forall \bar{J} \in \bar{\mathbb{J}}^k$. 
%	 This cut condition is equivalent to the pruning done in Algorithm \ref{alg1} in Step \ref{alg1-cut2} pointwise. As this pruning condition holds for the $\tilde{\theta}$, the online tree is cut in this node with the resulting $\tilde{\kappa}^k$. However, in the parametric analysis, as the comparison does not hold in the whole domain, the offline tree is not cut which results in exploring more nodes and consequently solving more QP relaxations. Therefore, the certification analysis tree will never be cut less than the online solver. The complexity measure for $\tilde{\theta}$ then increases by solving more relaxations in the offline analysis, i.e., $\tilde{\kappa}^{off} \geq \tilde{\kappa}^k$. 	
%	
%	%%%%%%%%%%%%%% 
%	Although the analysis may explore more nodes that have been already cut off in the online solver, the upper bound remains the same for all parameters in the offline tree in compare to the online tree. 
%	The reason is the extra nodes that might be explored are more restrictive, since more equality constraints are imposed. As the upper bound only is updated if a better integer solution is found, this implies that the parametric upper bound never will be updated and changed for $\tilde{\theta}$ in any extra nodes that
%	the analysis might explore compared to the online solver. In other words, the potential extra nodes seen will never improve the upper bound. See Section IV.A. of  \cite{axehill2010improved}. 
%	Therefore, for a single point the QP relaxations that are considered in Algorithm 2 will be a superset of the QP relaxations that would be solved in Algorithm 1. This in turn means that the total complexity returned by Algorithm 2 will be an upper bound on the total complexity of Algorithm 1 (pointwise) which makes the method conservative.  %\qed %, i.e.,  $\kappa^i_{tot} \geq \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i, \forall i$. \qed
%	%
%	%Because of the nodes that might have been previously cut off when the analysis and the on-line solver reaches the same arbitrary node, the on-line solver has explored a (correctly ordered) subset of the nodes that the analysis method has explored so far.
%	\end{proof}	
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	%
%	%	\begin{corollary} \label{cor-conserve-cert}	%(Complexity certificates): 
%	%	Let $\kappa(\theta)$ be a complexity measure for solving the QP relaxation $\mathcal{P}(\theta)$ returned by $\textsc{QPcertification} \left ( \mathcal{P}(\theta),\Theta \right )$ and that it satisfies $\kappa^j = \kappa(\theta)$, $\forall \theta\in \Theta^j \subseteq \Theta $, $\forall j$. Moreover, let $\{\Theta^i, \kappa^i_{tot} \}_{i}$ be the collection of tuples in  $\mathcal{F}$ returned by Algorithm \ref{alg2} and let $\kappa^*_{tot}(\theta)$ be the total complexity for solving all QP relaxations encountered in Algorithm \ref{alg1} for $\theta \in \Theta_0 $. Then $\kappa^i_{tot} \geq \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$.
%	%	\end{corollary}
%	%	\begin{proof} \label{proof-cor-conserve-cert}   
%	%	It immediately results from Theorem \ref{theorem-exact} and Theorem \ref{theorem-conservative}, such that in the actual PPWQ function comparisons, based on Theorem \ref{theorem-exact} , $\kappa^i_{tot} = \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$ whereas based on Theorem \ref{theorem-conservative}, $\kappa^i_{tot} \geq \kappa^*_{tot}(\theta)$, $\forall \theta\in \Theta^i$, otherwise. %\qed
%	%	\end{proof}
%
%	%%%%%%%%%%%%%%%%%%%%%%%
%	As a result, by approximate comparison, there might be a non-zero gap between the online complexity with the one provided from the analysis for a specific point, however all regions remain polyhedral which makes the computations significantly cheaper. So, there is a trade-off between computational time and the accuracy of the analysis. %Therefore 	
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{remark} \label{remark:infeas-cert}   
	In the analysis, we take the complexity measure resulted from the infeasible subproblem, that is the computation requires to find out a subproblem is infeasible, into account. Since, we are interested in finding the worst-case computation load that might need to be performed in finding the optimal integer solution in online solver. This provides a reliability of the certification method. 
	\end{remark}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	Although Algorithm \ref{alg2} applies Algorithm \ref{alg1} to all parameters simultaneously, it involves more complicated operations. On line \ref{alg2_cert}, Algorithm \ref{alg2} applies mp-QP certification parametrically instead of solving the problem only for a single parameter. Testing the cut conditions in Algorithm \ref{alg2} are performed parametrically, e.g., in Step \ref{alg2_comp}, two PPWQ functions are compared rather than comparing two single values as in Step \ref{alg1-cut2} of Algorithm \ref{alg1}. In general, the certification method predicts what would the online solver do for each certain parameter in the parameter set. 
	%TODO: this paragraph can be removed
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Don't remove the below lines!
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

